Splicing ViT Features for Semantic Appearance Transfer

We present a method for semantically transferring the visual appearance of one natural image to another. Specifically, our goal is to generate an image in which objects in a source structure image are "painted" with the visual appearance of their semantically related objects in a target appearance image. Our method works by training a generator given only a single structure/appearance image pair as input. To integrate semantic information into our framework - a pivotal component in tackling this task - our key idea is to leverage a pre-trained and fixed Vision Transformer (ViT) model which serves as an external semantic prior. Specifically, we derive novel representations of structure and appearance extracted from deep ViT features, untwisting them from the learned self-attention modules. We then establish an objective function that splices the desired structure and appearance representations, interweaving them together in the space of ViT features. Our framework, which we term "Splice", does not involve adversarial training, nor does it require any additional input information such as semantic segmentation or correspondences, and can generate high-resolution results, e.g., work in HD. We demonstrate high quality results on a variety of in-the-wild image pairs, under significant variations in the number of objects, their pose and appearance.

==> teaser.tex <==
\twocolumn[{
\renewcommand\twocolumn[1][]{#1}
\maketitle
\centering
\vspace*{-8.4cm}
\includegraphics[width=1\textwidth]{figures/teaser.pdf}
\captionof{figure}{Given two input images---a source \emph{structure} image and a target \emph{appearance} image--our method generates a new image in which the structure of the source image is preserved, while the visual appearance  of the target image is transferred in a \emph{semantically} aware manner. 
That is, objects in the structure image are ``painted'' with the visual appearance of semantically related objects in the appearance image. Our method leverages a self-supervised, pre-trained ViT model as an external semantic prior. This allows us to train our generator only on a single input image pair, without any additional information (e.g., segmentation/correspondences), and without adversarial training. Thus, our framework can work across a variety of objects and scenes, and can generate high quality results in high resolution (e.g., HD).
}\label{fig:teaser}
 \vspace*{0.25cm}
}]






% \twocolumn[{%
% \renewcommand\twocolumn[1][]{#1}%
% \maketitle
% %\begin{figure}[t]
% \vspace{-3.1in}
% %\centering
% \begin{minipage}{\textwidth}
% 	\centering
% \vspace*{-0.3cm}
% \includegraphics[width=1\textwidth]{figures/teaser_reduced.pdf}
% \captionof{figure}{Given two input images---a target \emph{texture} image and a source \emph{shape} image--our method generates a new image in which the shape of the source image is preserved while the texture from the target image is transferred in a semantically aware manner. Our method leverages a pre-trained Vision Transformer model as an external semantic prior, which allows us to train our generator only on a single texture/shape image pair, without any additional inputs (e.g., segmentation), and without adversarial training. \tali{add a sentence maybe about resolution and run-time?} }
% \label{fig:teaser}
% \end{minipage}
% %\afterfigure
% %\end{figure} 
% \vspace*{-1.5cm}
% }]

